Lost in Disclosure: On The Inference of Password Composition Policies

Large-scale password data breaches are becoming increasingly commonplace, which has enabled researchers to produce a substantial body of password security research utilising real-world password datasets, which often contain numbers of records in the tens or even hundreds of millions. While much study has been conducted on how password composition policies (sets of rules that a user must abide by when creating a password) influence the distribution of user-chosen passwords on a system, much less research has been done on inferring the password composition policy that a given set of user-chosen passwords was created under. In this paper, we state the problem with the naive approach to this challenge, and suggest a simple approach that produces more reliable results. We also present pol-infer, a tool that implements this approach, and demonstrates its use in inferring password composition policies.

==> _scraps.tex <==
% ROCKYOU LENGTHS TABLE
% =====================

\begin{table}[ht]
    \centering
    \caption{Frequencies $f(l)$ of passwords of different lengths $l$ in the RockYou set \cite{cubrilovich2009rockyou}, alongside their cumulative frequencies $cum(l)$ and the multiplier $mult(l)$ required to reach the frequency of the next length $f(l+1)$.}
    \begin{tabular}[c]{|l|l|l|l|}
        \hline
        $l$ & $f(l)$  & $cum(l)$ & $mult(l)$ \\ \hline
        1   & 314     & 314      & 4.32   \\ \hline % 4.318471337579618
        2   & 1042    & 1356     & 6.00   \\ \hline % 5.959439528023599
        3   & 6725    & 8081     & 9.72   \\ \hline % 9.724910283380769
        4   & 70506   & 78587    & 17.89  \\ \hline % 17.88529909527021
        5   & 1326965 & 1405552  & 7.03   \\ \hline % 7.039201680193973
        6   & 8488412 & 9893964  & 1.64   \\ \hline % 1.6355406185023516
        7   & 6288016 & 16181980 & ---    \\ \hline % 1.402487767257159
    \end{tabular}
    \label{tbl:rockyou-length}
\end{table}

% YAHOO LENGTHS TABLE
% ===================

\begin{table}[ht]
    \centering
    \caption{Frequencies $f(l)$ of passwords of different lengths $l$ in the Yahoo set \cite{gross2012yahoo}, alongside their cumulative frequencies $cum(l)$ and the multiplier $mult(l)$ required to reach the frequency of the next length $f(l+1)$.}
    \begin{tabular}[c]{|l|l|l|l|}
        \hline
        $l$ & $f(l)$  & $cum(l)$ & $mult(l)$ \\ \hline
        1   & 115     & 115      & 1.57   \\ \hline % 1.5739130434782609
        2   & 66      & 181      & 2.67   \\ \hline % 2.6685082872928176
        3   & 302     & 483      & 6.68   \\ \hline % 6.683229813664596
        4   & 2745    & 3228     & 2.65   \\ \hline % 2.6486988847583643
        5   & 5322    & 8550     & 10.31  \\ \hline % 10.313099415204679
        6   & 79627   & 88177    & 1.74   \\ \hline % 1.7440489016410174
        7   & 65608   & 153785   & ---    \\ \hline
    \end{tabular}
    \label{tbl:yahoo-length}
\end{table}

% YAHOO DIGITS TABLE
% ==================

\begin{table}[ht]
    \centering
    \caption{Frequencies $f(d)$ of passwords containing different numbers of digits $d$ in the yahoo set \cite{gross2012yahoo}, alongside their cumulative frequencies $cum(d)$ and the multiplier $mult(d)$ required to reach the frequency of the next length $f(d+1)$.}
    \begin{tabular}[c]{|l|l|l|l|}
        \hline
        $l$ & $f(l)$  & $cum(l)$ & $mult(l)$ \\ \hline
        0   & 156161  & 156161   & 1.40   \\ \hline % 1.4060538370186055
        1   & 56035   & 212196   & 1.13   \\ \hline % 1.1335237080161817
        2   & 86163   & 298359   & 1.15   \\ \hline % 1.1504685139134883
        3   & 39838   & 338197   & 1.03   \\ \hline % 1.0348073043165376
        4   & 50888   & 389085   & 1.07   \\ \hline % 1.067449357719781
        5   & 13543   & 402628   & 1.02   \\ \hline % 1.0161871633491164
        6   & 27157   & 429785   & 1.02   \\ \hline % 1.0241767450806196
        7   & 6957    & 429785   & ---    \\ \hline
    \end{tabular}
    \label{tbl:yahoo-digits}
\end{table} 

% 000WEBHOST LENGTHS TABLE
% ========================

\begin{table}[ht]
    \centering
    \caption{Frequencies $f(l)$ of passwords of different lengths $l$ in the 000webhost set \cite{osborne2015000webhost}, alongside their cumulative frequencies $cum(l)$ and the multiplier $mult(l)$ required to reach the frequency of the next length $f(l+1)$.}
    \begin{tabular}[c]{|l|l|l|l|}
        \hline
        $l$ & $f(l)$  & $cum(l)$ & $mult(l)$ \\ \hline
        1   & 306     & 306      & 6.03   \\ \hline % 6.0326797385620915032679738562092
        2   & 1540    & 1846     & 1.42   \\ \hline % 1.4198266522210184182015167930661
        3   & 775     & 2621     & 1.47   \\ \hline % 1.4658527279664250286150324303701
        4   & 1221    & 3842     & 1.66   \\ \hline % 1.6626756897449245184799583550234
        5   & 2456    & 6388     & 137.23 \\ \hline % 137.22557921102066374452097683156
        6   & 870209  & 876597   & 2.38   \\ \hline % 2.378161230303092527124779117428
        7   & 1208092 & 2084689  & ---    \\ \hline
    \end{tabular}
    \label{tbl:000webhost-length}
\end{table}

% 000WEBHOST DIGITS TABLE
% =======================

\begin{table}[ht]
    \centering
    \caption{Frequencies $f(d)$ of passwords containing different numbers of digits $d$ in the 000webhost set \cite{osborne2015000webhost}, alongside their cumulative frequencies $cum(d)$ and the multiplier $mult(d)$ required to reach the frequency of the next length $f(d+1)$.}
    \begin{tabular}[c]{|l|l|l|l|}
        \hline
        $d$ & $f(d)$  & $cum(d)$ & $mult(d)$ \\ \hline
        0   & 225024  & 255024   & 10.00     \\ \hline % 9.978488299140473
        1   & 2289730 & 2544754  & 2.30      \\ \hline % 2.304489549873976
        2   & 3319605 & 5864359  & 1.62      \\ \hline % 1.6151724340204956
        3   & 3607592 & 9471951  & 1.28      \\ \hline % 1.2767244045075825
        4   & 2621120 & 12093071 & 1.05      \\ \hline % 1.050397041413219
        5   & 609455  & 12702526 & 1.10      \\ \hline % 1.0921489158927917
        6   & 1170524 & 13873050 & 1.03      \\ \hline % 1.0256361794991007
        7   & 355652  & 14228702 & ---       \\ \hline
    \end{tabular}
    \label{tbl:000webhost-digits}
\end{table}

% OLD UPPER CONSTRAINTS INFERENCE SECTION
% =======================================

\subsubsection{Inferring Upper Constraints} The RockYou set is unique amongst those studied in this work for the upper limit of 0 it enforces on the number of non-alphanumeric characters (i.e. \textit{symbols}) passwords may contain. With only a slight modification to our approach, we can detect this class of constraint also (see Table~\ref{tbl:rockyou-symbols-desc}).

\begin{table}[ht]
\centering
\caption{Frequencies $f(s)$ of passwords containing different numbers of symbols $s$ in the RockYou set \cite{cubrilovich2009rockyou}, alongside their inverse cumulative frequencies $cum'(s)$ and the divisor $div(l)$ required to reach the frequency of the next symbol count $f(s+1)$.}
\label{tbl:rockyou-symbols-desc}
\begin{tabular}{|l|l|l|l|}
\hline
$s$ & $f(s)$   & $cum'(s)$ & $div(s)$ \\ \hline
0   & 31363674 & 32603048  & 26.31    \\ \hline % 26.306060963034565
1   & 914816   & 1239374   & 3.82     \\ \hline % 3.818651828024575
2   & 213432   & 324558    & 2.92     \\ \hline % 2.9206306354948435
3   & 59368    & 111126    & 2.15     \\ \hline % 2.147030410757757
4   & 25033    & 51758     & 1.94     \\ \hline % 1.936688493919551
5   & 6216     & 26725     & 1.30     \\ \hline % 1.3030864498512849
6   & 8278     & 20509     & 1.68     \\ \hline % 1.67680484016s2484
7   & 2526     & 12231     & ---      \\ \hline 
\end{tabular}
\end{table}

Our modified approach is identical to that shown in Section~\ref{sec:methodology}, but we instead use an inverse cumulative frequency $cum'(s)$ and a divisor $div(s)$ instead of a multiplier to reach the frequency of the next symbol count $f(s+1)$. That is to say, in Table~\ref{tbl:rockyou-symbols-desc}:

\begin{equation*}
    cum'(s + 1) = \frac{cum'(s)}{div(s)}
\end{equation*}

We can find the upper limit By taking $s$ where:

\begin{equation*}
    div(s) = max(\{div(m) | m \in \mathbb{N}\})
\end{equation*}

\begin{figure}[ht]
    \centering
    \includegraphics[width=\columnwidth]{figures/pdf/rockyou_symbols_desc_scatter.pdf}
    \caption{Frequencies $f(s)$ of passwords containing different numbers of symbols $s$ in the RockYou set \cite{cubrilovich2009rockyou}, plotted against the divisor $div(l)$ required to reach the frequency of the previous symbol count $f(s-1)$.}
    \label{fig:rockyou-symbols-desc}
\end{figure}

The outlying point at $s = 0$ in Figure~\ref{fig:rockyou-symbols-desc} indicates that the password composition policy that most of the passwords in the set were created under enforces a maximum number of non-alphanumeric symbols of $0$ (i.e. symbols are prohibited). This aligns with existing literature \cite{mayer2017second}.

% OLD SINGLES PADDED LINKEDIN 2WORD12 LENGTHS
% ===========================================

\begin{table}[ht]
\centering
\caption{Lorem.}
\label{tbl:synth-padded-length}
\begin{tabular}{|l|l|l|l|}
\hline
$l$ & $f(l)$  & $cum(l)$  & $mult(l)$ \\ \hline
1   & 5       & 5         & 3.40      \\ \hline % 3.4
2   & 12      & 17        & 6.47      \\ \hline % 6.470588235294118
3   & 93      & 110       & 8.00      \\ \hline % 8.0
4   & 770     & 880       & 2.42      \\ \hline % 2.418181818181818
5   & 1248    & 2128      & 3.45      \\ \hline % 3.4473684210526314
6   & 5208    & 7336      & 1.52      \\ \hline % 1.5139040348964012
7   & 3770    & 11106     & 1.46      \\ \hline % 1.462992976769314
8   & 5142    & 16248     & 1.00      \\ \hline % 1.0
9   & 0       & 16248     & 1.00      \\ \hline % 1.0
10  & 0       & 16248     & 1.00      \\ \hline % 1.0
11  & 0       & 16248     & 34.53     \\ \hline % 34.53452732644018
12  & 544869  & 561117    & 1.52      \\ \hline % 1.5188400993019282
13  & 291130  & 852247    & 1.24      \\ \hline % 1.235458734380995
14  & 200669  & 1052916   & ---       \\ \hline
\end{tabular}
\end{table}

% OLD SINGLES PADDED LINKEDIN 2WORD12 WORDS
% ===========================================

\begin{table}[ht]
\centering
\caption{Lorem.}
\label{tbl:synth-padded-words}
\begin{tabular}{|l|l|l|l|}
\hline
$w$ & $f(w)$  & $cum(w)$  & $mult(w)$ \\ \hline
0   & 1556    & 5         & 3.40      \\ \hline % 10.17159383033419
1   & 14271   & 5         & 3.40      \\ \hline % 68.75503885764832
2   & 1072359 & 17        & 6.47      \\ \hline % 1.1752687500114871
3   & 190725  & 110       & 8.00      \\ \hline % 1.070230844835958
4   & 89819   & 880       & 2.42      \\ \hline % 1.0382946234830828
5   & 52415   & 2128      & 3.45      \\ \hline % 1.0254513086279022
6   & 36170   & 7336      & 1.52      \\ \hline % 1.0125950806791943
7   & 18355   & 11106     & ---       \\ \hline
\end{tabular}
\end{table}

